Sticker-TTS: Learn to Utilize Historical Experience with a Sticker-driven Test-Time Scaling Framework

Large reasoning models (LRMs) have exhibited strong performance on complex reasoning tasks, with further gains achievable through increased computational budgets at inference. However, current test-time scaling methods predominantly rely on redundant sampling, ignoring the historical experience utilization, thereby limiting computational efficiency. To overcome this limitation, we propose Sticker-TTS, a novel test-time scaling framework that coordinates three collaborative LRMs to iteratively explore and refine solutions guided by historical attempts. At the core of our framework are distilled key conditions-termed stickers-which drive the extraction, refinement, and reuse of critical information across multiple rounds of reasoning. To further enhance the efficiency and performance of our framework, we introduce a two-stage optimization strategy that combines imitation learning with self-improvement, enabling progressive refinement. Extensive evaluations on three challenging mathematical reasoning benchmarks, including AIME-24, AIME-25, and OlymMATH, demonstrate that Sticker-TTS consistently surpasses strong baselines, including self-consistency and advanced reinforcement learning approaches, under comparable inference budgets. These results highlight the effectiveness of sticker-guided historical experience utilization. Our code and data are available at https://github.com/RUCAIBox/Sticker-TTS.

==> prompts/extractor.tex <==
Given the solution provided below, Generate an abstract of the key conditions that help solve the problem. The abstract should include both the key conditions and the question.

Abstract Format:

**Conditions:**

1. [Condition 1]

2. [Condition 2]

... (add more conditions as needed)

**Question:**

[Clearly state what is being asked.]

Requirements:

1. **Conditions**

   - Only retain the key steps that directly impact solving the problem, ignoring lengthy derivations and irrelevant calculations.
   
   - Each step must have a clear mathematical significance, meaning it makes a substantial contribution to the final conclusion.
   
   - The conditions can come from the reasoning process.
   
   - Write each condition on a separate line, numbered sequentially.
   
   - Remove repetitive calculations and obvious equation transformations.
   
   - **List as many conditions as possible**
   
   - **Do not record direct substitutions of common formulas unless they play a key role in the derivation.**
   
   - **Each condition must be atomic and indivisible** (i.e., it cannot be divided into two sub-conditions).
   
   - **Each condition must refer to something clearly and without ambiguity.**!!!

2. **Question:**

   - Summarize what is being asked in one clear sentence.
   
   - Remove all known conditions.


solution to question:

[Solution]

Please provide your output strictly following the abstract format without other unnecessary words.

==> sections/3-Empirical_Study.tex <==
\section{Empirical Study}
\label{sec:empirical_study}
In this section, we conduct empirical studies to analyze how to improve the retrieval and reasoning capabilities of LLMs for multi-document question answering from three aspects, \ie performance gap, evidence selection, and attention intervention.

% \subsection{Performance Gap: Gold Evidence vs. Long-Context Retrieval}
\subsection{Performance Gap}
\label{sec:performance_gap}
We first explore how the additional documents effect the final performance in the long context. We compare the performance of LLMs from inputting only gold evidence documents to gradually insert more distracting documents. We show the results in Figure~\ref{fig:exp-gold-other}. 
We can observe that as the number of irrelevant documents increases and the input becomes longer, the performance of the model significantly deteriorates. This indicates that in the case of long inputs, the model's retrieval and reasoning abilities have significantly declined due to the interference of large irrelevant information. 
Inspired by this, we hope to design a retrieval strategy to filter out the irrelevant documents in long inputs. 

\subsection{Evidence Selection}
\label{sec:evidence_selection}

In this study, we examine document retrieval in multi-document QA using two primary methods: in-context retrieval and attention-based retrieval. The in-context retrieval method prompts LLMs to directly select the top-\(k\) documents most relevant to the given question, while attention-based retrieval method utilizes the attention distribution over each document to perform selection. Subsequently, the selected documents are employed as condensed input in the question-answering prompt. The results, presented in Table~\ref{tab:recall-icr-attention}, demonstrate that the attention-based approach significantly outperforms the in-context retrieval method, particularly as document length increases (e.g., recall score decreases by 50.6\% on HotpotQA-32K).  


\begin{table}[htbp]
  \centering
  \small
  \begin{tabular}{lc}
    \toprule
    \textbf{Mask Mode} & \textbf{SubEM} \\
    \midrule
    No Mask & \textbf{60.5} \\
    % Closed Book & 23.0 \\
    $\text{Evidence}_{2}$ $\rightarrow$ $\text{Evidence}_{1}$ & 60.0 \\
    Question $\rightarrow$ $\text{Evidence}_{1}$ & 48.0 \\
    Question $\rightarrow$ $\text{Evidence}_{2}$ & 42.0 \\
    Question $\rightarrow$ $\text{Evidence}_{1}$, $\text{Evidence}_{2}$ & 29.5 \\
    \bottomrule
  \end{tabular}
  \caption{SubEM scores on HotpotQA-8K with various masking strategies using Llama-3.1-8B-Instruct, where \(\text{Evidence}_{1}\) and \(\text{Evidence}_{2}\) refer to the first and second gold documents in the context.}
  \label{tab:attention-flow}
\end{table}


\subsection{Attention Intervention}\label{sec:attention_intervention}
Through the above experiments, we find that using attention heads can effectively help the model to retrieve the most relevant documents from long inputs. In this section, we further explore how to facilitate the model's utilization of multiple retrieved documents. Specifically, we select some questions from HotpotQA that require the use of two gold documents for answering within 8K length. Based on the attention interaction, we mask the attention between the two gold documents, as well as mask the attention of the questions to the two gold documents, respectively. We show the results in Table~\ref{tab:attention-flow}. First, masking the attention between the two gold documents has negligible impact on performance compared to the unmasked condition (60.0\% for Evidence$_2$ $\rightarrow$ Evidence$_1$ vs. 60.5\% for No Mask). This suggests that during multi-hop question-answering, the LLM does not engage in implicit reasoning while encoding long inputs, aligning with observations from recent studies~\cite{yu-emnlp-2024-incontext}. Additionally, masking the attention from the question to any gold document results in a significant performance drops. When all gold documents are masked simultaneously, the SubEM score even decreases to a level similar to that observed when no document is provided (29.5\% for Question $\rightarrow$ $\text{Evidence}_{1}$, $\text{Evidence}_{2}$ vs. 23.0\% for Closed Book). This demonstrates that the directly attention from the question to the gold documents plays a critical role in the LLM's overall performance. 

Building on the preceding experiments, attention heads can be employed to assist the LLM in retrieving pertinent documents from long inputs. In addition, By adjusting the attention directed towards these documents, the model's ability to utilize them in answering questions is enhanced. These principles will guide the design of our method.
